Towards reduction of Paradigm coordination models

The coordination modelling language Paradigm addresses collaboration between components in terms of dynamic constraints. Within a Paradigm model, component dynamics are consistently specified at a detailed and a global level of abstraction. To enable automated verification of Paradigm models, a translation of Paradigm into process algebra has been defined in previous work. In this paper we investigate, guided by a client-server example, reduction of Paradigm models based on a notion of global inertness. Representation of Paradigm models as process algebraic specifications helps to establish a property-preserving equivalence relation between the original and the reduced Paradigm model. Experiments indicate that in this way larger Paradigm models can be analyzed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{L. Aceto and M.R. Mousavi (Eds.): PACO 2011\\
EPTCS 60, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.60.1}{10.4204/EPTCS.60.1}}

